HPAC-ML: A Programming Model for Embedding ML Surrogates in Scientific Applications

Recent advancements in Machine Learning (ML) have substantially improved its predictive and computational abilities, offering promising opportunities for surrogate modeling in scientific applications. By accurately approximating complex functions with low computational cost, ML-based surrogates can accelerate scientific applications by replacing computationally intensive components with faster model inference. However, integrating ML models into these applications remains a significant challenge, hindering the widespread adoption of ML surrogates as an approximation technique in modern scientific computing. We propose an easy-to-use directive-based programming model that enables developers to seamlessly describe the use of ML models in scientific applications. The runtime support, as instructed by the programming model, performs data assimilation using the original algorithm and can replace the algorithm with model inference. Our evaluation across five benchmarks, testing over 5000 ML models, shows up to 83.6x speed improvements with minimal accuracy loss (as low as 0.01 RMSE).

==> latexmkrc <==
#!/usr/bin/env perl
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -i dvipdfmx-unsafe.cfg -o %D %O %S";

# Workaround to allow pstricks transparency (https://github.com/overleaf/issues/issues/3449)
$dvipdf = "dvipdf -dNOSAFER -dALLOWPSTRANSPARENCY %O %S %D";

###############################
# Post processing of pdf file #
###############################

$compiling_cmd = "internal overleaf_pre_process %T %D";
$success_cmd = "internal overleaf_post_process %T %D";
$failure_cmd = $success_cmd;

# equivalent to -gt option. Used to prevent latexmk from skipping recompilation
# of output.log and output.pdf
$go_mode = 3;

# equivalent to -bibtex option. Run bibtex unconditionally when bbl files are
# out of date.
$bibtex_use = 2;

my $ORIG_PDF_AGE;

sub overleaf_pre_process {
    my $source_file = $_[0];
    my $output_file = $_[1];

    # get age of existing pdf if present
    $ORIG_PDF_AGE = -M $output_file
}

sub overleaf_post_process {
    my $source_file = $_[0];
    my $output_file = $_[1];
    my $source_without_ext = $source_file =~ s/\.tex$//r;
    my $output_without_ext = $output_file =~ s/\.pdf$//r;

    # Look for a knitr concordance file
    my $concordance_file = "${source_without_ext}-concordance.tex";
    if (-e $concordance_file) {
        print "Patching synctex file for knitr...\n";
        system("patchSynctex.R", $source_without_ext, $output_without_ext);
    }

    # Return early if pdf file doesn't exist or wasn't updated
    my $NEW_PDF_AGE = -M $output_file;
    return if !defined($NEW_PDF_AGE);
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE;

    # Figure out where qpdf is
    $qpdf //= "/usr/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf;
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});

    # Run qpdf
    my $optimised_file = "${output_file}.opt";
    system($qpdf, split(' ', $qpdf_opts), $output_file, $optimised_file);
    $qpdf_exit_code = ($? >> 8);
    print "qpdf exit code=$qpdf_exit_code\n";

    # Replace the output file if qpdf was successful
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($qpdf_exit_code == 0 || $qpdf_exit_code == 3);
    print "Renaming optimised file to $output_file\n";
    rename($optimised_file, $output_file);

    print "Extracting xref table for $output_file\n";
    my $xref_file = "${output_file}xref";
    system("$qpdf --show-xref ${output_file} > ${xref_file}");
    $qpdf_xref_exit_code = ($? >> 8);
    print "qpdf --show-xref exit code=$qpdf_xref_exit_code\n";
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
add_cus_dep( 'Rtex', 'tex', 0, 'do_knitr');
add_cus_dep( 'Rnw', 'tex', 0, 'do_knitr');
sub do_knitr {
    Run_subst(qq{Rscript -e '
        library("knitr");
        opts_knit\$set(concordance=T);
        knitr::knit(%S, output=%D);
        '}
    );
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############

sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/local/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}

